Data Readiness for AI: A 360-Degree Survey

Artificial Intelligence (AI) applications critically depend on data. Poor quality data produces inaccurate and ineffective AI models that may lead to incorrect or unsafe use. Evaluation of data readiness is a crucial step in improving the quality and appropriateness of data usage for AI. R&D efforts have been spent on improving data quality. However, standardized metrics for evaluating data readiness for use in AI training are still evolving. In this study, we perform a comprehensive survey of metrics used to verify data readiness for AI training. This survey examines more than 140 papers published by ACM Digital Library, IEEE Xplore, journals such as Nature, Springer, and Science Direct, and online articles published by prominent AI experts. This survey aims to propose a taxonomy of data readiness for AI (DRAI) metrics for structured and unstructured datasets. We anticipate that this taxonomy will lead to new standards for DRAI metrics that will be used for enhancing the quality, accuracy, and fairness of AI training and inference.

==> sections/drai.tex <==
In this section, we examine the concept of data readiness for AI and explore the processes involved in preparing data for effective AI usage. Furthermore, we will discuss the significance of assessing data readiness for AI, emphasizing the importance of robust frameworks, methodologies, and metrics to evaluate and enhance the suitability of data for AI applications. By addressing the key challenges and considerations in data readiness, organizations can lay a solid foundation for AI implementation and unlock the full potential of their data resources.

\vspace{-12pt}
\subsection{Processes of Readying Data for AI}
\label{sec:drai-process}
%This section focuses on exploring the various processes involved in preparing data for AI, shedding light on the importance of data quality, data preprocessing techniques, and feature engineering methods. By examining these fundamental aspects, we aim to provide a comprehensive overview of the practices and challenges associated with data readiness for AI, offering valuable insights to researchers, practitioners, and organizations striving to maximize the potential of AI in their respective domains.

The AI 
%data readiness 
community defines the processes of readying data for AI as a series of steps aimed at preparing the data to be suitable for machine learning and AI applications. 
According to IBM 
Biddle et al. \cite{biddle2023prepare} describe that data preparation for AI involves transforming data into a format suitable for model development, measurement, and training. This includes processes such as selecting relevant features, merging data sets, deriving new features, formatting, sorting the data, addressing missing values, and ensuring data accuracy and completeness.
In parallel, Informatica \cite{Tawfik_Hanthur_Sanyal_2021} emphasizes critical processes in data preparation for AI projects. These processes include finding and accessing trusted data, analyzing data lineage and relationships, preparing and cleansing the data, enriching the data through feature engineering or incorporating additional data, and implementing the data pipeline for reuse and automation. Similarly, Lawton \cite{Lawton_2022} characterizes data preparation as a time-consuming and complex process. It involves various processes such as problem formulation, data collection, data exploration, data cleansing and validation, data structuring, feature engineering, and feature selection. These processes collectively aim to ensure accurate and adaptable algorithms, ultimately saving time and effort for data scientists and business users.

To further enhance the quality, relevance, and usability of data for AI and machine learning applications, AltexSoft \cite{Editor_2020} outlines ten fundamental processes for preparing datasets. These processes incorporate problem articulation, establishing data collection mechanisms, assessing data quality, formatting data for consistency, reducing data, data cleaning, creating features, joining transactional and attribute data, rescaling data, and discretizing data.

In addition to these essential processes, the Data Readiness Report, as introduced by Afzal et al. \cite{afzal2020data}, plays an important role in readying data for AI. This report serves as documentation of operations conducted during data preparation, cleaning, and quality analysis. By providing insights into dataset characteristics and evaluating them against relevant quality dimensions, the Data Readiness Report effectively addresses data challenges upfront and contributes to the overall effectiveness of data preparation for AI applications.

Overall, the AI 
%data readiness 
community defines the processes of readying data for AI as a set of tasks that involve transforming, cleaning, validating, enriching, and documenting the data to make it suitable for model development, training, and analysis. These processes aim to ensure data readiness ultimately facilitating effective AI and machine learning outcomes.

% Interesting read to include in defining AI readiness section: https://atlan.com/know/ai-readiness/ai-ready-data/

\vspace{-12pt}
\subsection{Assessing Data Readiness}
\label{sec:drai-needs}
Assessing data readiness for AI is crucial for ensuring the performance, fairness, and reliability of AI systems. It involves evaluating quality, completeness, representativeness, and other data readiness dimensions, including feature relevancy, duplicity, class separability, FAIR (Findable, Accessible, Interoperable, and Reusable) principle compliance, and outliers used for training and deploying AI models. By conducting a thorough assessment, AI users can identify and address data readiness issues, mitigate bias and fairness concerns, improve model generalization and robustness, and comply with data governance and ethical guidelines. In addition, assessing data readiness in the early stages of the ML pipeline is highly beneficial. By evaluating data readiness at an early stage, organizations can identify any data-related challenges or limitations upfront, allowing for proactive measures and adjustments. In Fig. ~\ref{fig:DR4AI_ML_Pipeline}, we illustrate the placement of data readiness evaluation within the ML pipeline, emphasizing the importance of conducting these assessments early on.
Furthermore, during model evaluation, issues such as model bias or insufficient data quality might be detected. This necessitates a re-evaluation of data readiness to address these issues. By incorporating this iterative feedback loop, organizations can ensure continuous improvement of the data and model. Ultimately, assessing data readiness enhances AI systems' overall effectiveness and trustworthiness, enabling them to make accurate predictions and informed decisions in real-world applications.

\begin{figure}
  \centering
  %\includegraphics[width=0.75\textwidth]{images/ML Pipeline with DR4AI.png}
  \includegraphics[width=0.5\textwidth]{images/enhanced_ml_pipeline_data_readiness_crop.pdf}
  \caption{Enhanced ML pipeline with the evaluation of data readiness}
  \label{fig:DR4AI_ML_Pipeline}
\end{figure}

Assessing data readiness for AI applications is a multifaceted challenge, as discussed by Allen \cite{allen2019assessing} and Gupta et al. \cite{gupta2021data}. These approaches provide insights into various aspects of data readiness. On the one hand, Allen's article highlights five key dimensions: data accessibility, size, usability, understandability, and maintainability. It highlights the need for strategic data management, including external sources and adherence to good data practices. On the other hand, Gupta et al.'s toolkit offers a practical, automated approach to assessing data readiness and addressing data readiness challenges. It provides an array of readiness metrics for structured datasets, covering dimensions like completeness, accuracy, consistency, and timeliness. These metrics empower data scientists to understand data limitations and guide data preparation effectively. By merging these studies, there is potential for a comprehensive framework that improves data readiness in AI projects, including both strategic considerations and practical data readiness assessment techniques.

Data scientists often face challenges during the pre-processing stage, which can significantly impact productivity and introduce data readiness issues. These include dealing with missing or incomplete data, handling noisy or irrelevant features, addressing class imbalances in the dataset, ensuring data privacy and security, managing data scalability and storage constraints, handling unstructured or semi-structured data formats, and dealing with inconsistencies or errors in data sources. Afzal et al. \cite{afzal2020data} introduced the concept of a data readiness report seeking to address these challenges. This report provides detailed insights into the readiness of input data across various dimensions. It captures data properties, identifies quality issues, and documents data operations performed by different individuals involved in the data preparation process. Alongside Datasheets (Gebru et al. \cite{gebru2018datasheets}) and Model Cards (Mitchell et al. \cite{mitchell2019modelcards}), the data readiness report enhances transparency, documentation, and governance in the AI pipeline. It promotes responsible AI development by ensuring stakeholders have a clear understanding of the dataset's strengths, limitations, and suitability for training machine learning models.

To further enhance the assessment of data readiness for AI, Lawrence \cite{lawrence2017data} focuses on assessing data readiness by categorizing it into different bands (C, B, and A) based on accessibility, accuracy, representation, and appropriateness. Each band represents a specific level of data readiness for analysis or distribution. Band C focuses on data accessibility, requiring it to be made machine-readable and ethically handled. Band B emphasizes verifying data accuracy and representation, addressing missing values and errors. Band A considers the appropriateness of the dataset for specific tasks involving careful evaluation and potential annotation or new data collection. By categorizing data readiness into these bands, the framework provides a structured methodology for evaluating and improving data readiness, thereby enhancing the reliability and effectiveness of AI systems. 

Similar to Lawrence's \cite{lawrence2017data} work on data readiness, Harvey et al. \cite{Harvey2019} also addressed the topic by introducing the MIDaR (Medical Imaging Data Readiness) scale. It is a framework for assessing the readiness of medical imaging data for AI applications, considering FAIR (Findable, Accessible, Interoperable, and Reusable) principles and different stages of data preparation. It categorizes data into four levels: D, C, B, and A. Level D represents abundant but inaccessible and un-anonymized data. Level C indicates anonymized data with artifacts and noise. Level B signifies structured and quality-controlled data without labels, and Level A represents labeled and statistically powered data ready for AI tasks. As data progresses toward Level A, its value increases, although the volume may decrease. The MIDaR scale provides insights into data characteristics, ethics, labeling, and statistical power when preparing medical imaging data for AI analysis.

In line with the focus on data readiness assessment, Patel et al. \cite{Automatic:Patel} \cite{10.1145/3603709} emphasize the importance of systematically analyzing data characteristics to improve the efficacy of machine learning and artificial intelligence applications. Their research outlines the need for intelligently designed metrics and transformation operations that effectively address data readiness gaps, reducing the effort required for debugging in the machine learning pipeline. This perspective on data readiness aligns with the principles embedded in OpenDataVal introduced by Jiang et al. \cite{jiang2023opendataval}, an existing benchmark framework. OpenDataVal provides a unified environment for researchers and practitioners to apply and compare various data valuation algorithms. With a diverse collection of datasets, the implementation of state-of-the-art data valuation algorithms, and proposed machine learning tasks for evaluating data readiness, OpenDataVal significantly contributes to streamlining data preparation. The framework's integrated environment and prediction model API further facilitate the seamless integration of various models. This comprehensive approach in OpenDataVal aims to enhance machine learning outcomes by promoting robust data preparation and evaluation strategies.

\begin{table}[t]
\centering
\caption{Comparison of Data Readiness Assessment Approaches for AI Applications}
\label{tab:dr4ai-comparison}
\vspace{-10px}
\setlength\extrarowheight{2pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Reference}} &
  \multicolumn{1}{c|}{\textbf{Summary}} \\ \hline
Allen \cite{allen2019assessing} &
  \begin{tabular}[c]{@{}l@{}}Explores challenges and considerations in assessing data readiness for AI applications. \\ Focuses on data accessibility, size, usability, understandability, and maintainability. \\ Emphasizes the importance of data strategy, considering external sources, and following good data practices.\end{tabular} \\ \hline
Gupta et al.\cite{gupta2021data} &
  \begin{tabular}[c]{@{}l@{}}Presents a data quality toolkit for automated data readiness assessment.\\ Reduces preparation time and enhances data readiness. \\ Offers various readiness metrics for accessible and actionable assessment by diverse users.\\ Assists in identifying issues and guiding data cleansing and transformation.\end{tabular} \\ \hline
Afzal et al. \cite{afzal2020data} &
  \begin{tabular}[c]{@{}l@{}}Introduces the concept of a data readiness report. \\ Provides comprehensive documentation of data readiness across dimensions. \\ Captures data properties, readiness issues, and operations during data preparation. \\ Enhances transparency, documentation, and governance in the AI pipeline.\end{tabular} \\ \hline
Lawrence \cite{lawrence2017data} &
  \begin{tabular}[c]{@{}l@{}}Categorizes data readiness into bands (C, B, and A) based on accessibility, accuracy, representation, and appropriateness. \\ Each band represents a specific level of data readiness for analysis or distribution.\end{tabular} \\ \hline
Harvey et al. \cite{Harvey2019} &
  \begin{tabular}[c]{@{}l@{}}Introduces the MIDaR scale for assessing medical imaging data readiness for AI applications. \\ Considers FAIR principles and data preparation stages.   \\ Categorizes data into four levels (D, C, B, and A) based on data characteristics, ethics, labeling, and statistical power.\end{tabular} \\ \hline
Patel et al. \cite{Automatic:Patel} \cite{10.1145/3603709} &
  \begin{tabular}[c]{@{}l@{}}Highlights the importance of systematically analyzing data readiness to improve AI application efficacy. \\ Provides intelligently designed metrics and transformation operations for addressing data readiness gaps. \\ Reduces debugging effort in the machine learning pipeline.\end{tabular} \\ \hline
Jiang et al. \cite{jiang2023opendataval} &
  \begin{tabular}[c]{@{}l@{}}OpenDataVal creates a unified framework where practitioners can employ and compare diverse data valuation algorithms \\ Offer a broad range of datasets, implementing data valuation algorithms, and defining machine learning tasks for assessing data readiness. \end{tabular} \\ \hline
\end{tabular}%
}
\vspace{-10px}
\end{table}

In Table \ref{tab:dr4ai-comparison}, we compare various AI readiness approaches discussed in this section. Evaluating data readiness for AI is crucial for robust and reliable machine learning systems. This process -- including data characteristics, completeness, representativeness, and more -- aids in addressing issues, reducing biases, enhancing model performance, and ensuring ethical compliance. The complexities involved emphasize the need for a strong data strategy, exploration of external data sources, and robust data pipelines. The advent of assessment frameworks and toolkits empowers practitioners to improve the trustworthiness of AI systems. Ongoing research in data readiness will contribute to responsible AI deployment, enabling accurate decisions across diverse applications. Prioritizing data readiness establishes a good foundation for AI success, promoting transparency, accountability, and responsible development.



==> sections/related_work.tex <==
%In this section, we present a comprehensive overview of prior research, with a specific focus on data readiness metrics for both structured and unstructured data. Data readiness is crucial for AI models to ensure accurate and reliable results. Our goal is to examine various studies and metrics, providing a comprehensive understanding of how to evaluate data readiness effectively. This knowledge will lead to better AI implementations that are both effective and responsible.

Toward gaining an understanding of metrics for AI data readiness, a small number of studies surveyed data preprocessing stages in preparing data for AI. Priestley et al. \cite{article:priestley} conducted a significant study highlighting the critical role of decision-makers and practitioners in improving data-focused practices. They highlighted the significance of data cleaning and preprocessing stages, including feature selection, duplicate elimination, outlier removal, consistency assurance, and handling of missing values. Documentation of these preprocessing steps was essential to ensure compatibility and identify potential dependencies and information leakages among features. Their insights, derived from an extensive literature survey, laid the foundation for recognizing the pivotal role of data readiness in AI applications. 
Yalaoui et al. \cite{9678209} presented a survey paper specifically focused on data quality evaluation and enhancement. They compared existing frameworks, models, and methods for data quality evaluation and enhancement, and identified research directions and challenges. 
%By doing so, we aim to highlight existing metrics available in the literature that can help determine the readiness of data for AI.

%Our study goes beyond singular dimensions of data readiness by considering a comprehensive set of metrics for both structured and unstructured data. 
%For instance, 
There are a few studies that looked into metrics for unstructured data. Elmagarmid et al. \cite{4016511} explored into similarity metrics for duplicate record detection, specifically focusing on challenges posed by typographical variations in string data. Li et al. \cite{10.1145/3136625} concentrated on feature selection metrics, categorizing traditional approaches into wrapper methods, filter methods, embedded methods, and hybrid methods. Furthermore, Forman \cite{10.5555/944919.944974} explored feature selection metrics for text classification, examining their performance. 
%In our survey, we address a diverse range of critical data readiness aspects. By exploring multiple dimensions, our study provides a more comprehensive understanding of data readiness for AI applications. 
%Moreover, our study delves extensively into metrics specifically tailored for handling unstructured data, recognizing the growing importance of visual data in AI applications. 
The studies on image quality measures \cite{5412098} and perceptual visual quality metrics \cite{LIN2011297} are important in understanding data readiness for unstructured data, particularly in the context of visual data, where image quality assessment and perceptual metrics are essential for effective AI applications.

In the context of bias and fairness, Shahbazi et al. \cite{10.1145/3588433} provided a survey of techniques focused on identifying and mitigating representation bias across diverse data types, such as structured data, image data, textual data, and graph data. They discussed the problem definition, causes, and methods for measuring and quantifying representation bias in both structured and unstructured data. Addressing the issue of discrimination in data readiness for AI systems, Ntoutsi et al. \cite{ntoutsi2020bias} focused on the challenges and implications of biased data on the fairness and accuracy of AI-based decision-making. They emphasized the importance of understanding and mitigating biases in data to prevent the continuation of discriminatory practices. Similarly, in the context of privacy, Wagner et al. \cite{10.1145/3168389} reviewed over 80 privacy metrics across six domains categorizing them based on the aspect of privacy measured, required inputs, and data types needing protection. It identifies research gaps in areas such as metric combination and interdependent privacy, proposing a method for selecting appropriate metrics through nine key questions. Emphasizing the importance of employing multiple metrics to address diverse privacy aspects, the paper serves as a reference guide and toolbox for privacy researchers, aiding informed choices in metric selection for specific scenarios.
%Our study complements these findings by providing metrics and insights that play a crucial role in addressing discrimination and ensuring the suitability of data for AI applications. We highlight the importance of evaluating bias-related issues in data and promoting awareness among AI scientists and decision-makers.

Building upon existing comprehensive surveys, our study aims to contribute to the evolving field of data readiness metrics, with a specific focus on metrics for both structured and unstructured data. While previous works have explored specific dimensions or focused on individual metrics, we address the lack of a comprehensive study including numerous data readiness dimensions for AI applications. There are broader perspectives in addressing data readiness for AI applications. We identify numerous important factors that define data readiness, such as data preparation, privacy leakage evaluation, data discrimination evaluation, compliance to FAIR principles, mislabeled data detection, feature relevancy analysis, bias-related issues, and quality evaluation of speech and multimedia data. 
To survey existing literature in these dimensions and to identify gaps,
%proposing metrics for measuring data readiness, 
our effort aims to advance the AI data readiness field and inform best practices for evaluating the suitability of data for AI applications. Given the growing importance of data readiness, our study fills an important gap in the literature and provides valuable insights for practitioners and decision-makers in the field.

